An SDN-based Approach For Defending Against Reflective DDoS Attacks

Distributed Reflective Denial of Service (DRDoS) attacks are an immanent threat to Internet services. The potential scale of such attacks became apparent in March 2018 when a memcached-based attack peaked at 1.7 Tbps. Novel services built upon UDP increase the need for automated mitigation mechanisms that react to attacks without prior knowledge of the actual application protocols used. With the flexibility that software-defined networks offer, we developed a new approach for defending against DRDoS attacks; it not only protects against arbitrary DRDoS attacks but is also transparent for the attack target and can be used without assistance of the target host operator. The approach provides a robust mitigation system which is protocol-agnostic and effective in the defense against DRDoS attacks.

==> doc/evaluation.tex <==
% !TeX spellcheck = en_US
\section{Detection Evaluation}
\label{sec:eval}

%Our two-part evaluation consists of a reliability evaluation and a performance evaluation. For the reliability evaluation, we analyzed whether the algorithms behind the system can effectively identify DRDoS attacks while the performance evaluation determines whether it is possible to deploy the system in a production network with commodity hardware.

%\subsection{Reliability Evaluation}

\subsection{Data Set}

We use traffic traces of the MAWI Working Group Traffic Archive~\cite{mawilab}, more precisely, a recording of 48 hours of traffic in the backbone network of the WIDE project\footnote{https://www.wide.ad.jp/} from April 12th and April 13th of 2017. The amount of traffic in the network fluctuates between circa 50.000 and 150.000 packets per second, the amount of UDP traffic fluctuates between 6 to 9 percent of all traffic in the network.

\subsection{Test Design}

For our analyses, we split up the MAWI dataset in time frames of length $l$ and calculated the entropy values both for the benign traffic and for added attack traffic with magnitude $a$ for each time frame (where $a=1$ means that the attack contains as many flows as the benign traffic in the network).

\begin{figure*}
    \small
	\centering
	\includegraphics[width=\textwidth]{fig/sp-entropy-example.pdf}
	\caption{Source port entropy during two days of traffic without an attack and during simulated attack runs with attack magnitude $a$ in multiples of the benign UDP traffic ($l=300s$).}
	\label{fig:sp-entropy-ex}
\end{figure*}
One example output of such a test run can be seen in Figure~\ref{fig:sp-entropy-ex}. The figure shows changes in the source port entropy over 48 hour with and without attacks for a time frame length $l$ of 300s. 
We then use these entropy values as input for our detection algorithm described in Section~\ref{sec:detection}. Afterwards, we analyze whether an attack was detected for the benign traffic (false positive, FP), no attack was detected for benign traffic (true negative, TN), attacks were detected for traffic with added attack traffic (true positive, TP), or no attack was detected for traffic including attack traffic (false negative, FN). From there, over the whole data set of two days of traffic, precision $P = TP / (TP + FP)$, recall $R = TP / (TP + FN)$, and accuracy $A = (TP + TN)/(TP+TN+FP+FN)$ were calculated for all parameters in Table~\ref{tab:eval_params}. For each attack strength, we compare these values with the analysis of the benign traffic. Therefore, the data set is fully balanced in each test run; the amount of values with positive predicted condition is equal to the amount of values with negative predicted condition. 

\subsection{Results}

\begin{table}
	\centering
	\caption{Parameters for the classification reliability evaluation.}
	\label{tab:eval_params}
	\begin{tabular}{lll}
    Description & Name & Values \\
    \hline
    Entropy base & & Packets, flows\\
    Entropy combination & & Mean, median\\
    Classification threshold & $T_h$ & -0.5, -1, -1.5, -2, -2.5, -3, -3.5\\
    Ratio threshold & $T_r$ & 0.05, 0.1, 0.2, 0.25, 0.3, 0.35\\
    Gap size in frames & g & 5, 10, 60, 300 \\
    Frame length in seconds & l & 1s, 10s, 30s, 60s, 90s, 300s, 600s \\
    Amount of entropy values & e & 1, 2, 3, 4, 5\\
    Attack magnitude & $a$ & $0.5, 1, 1.5, 2, 2.5$\\
    Subnet size (dest. IP) & $s$ & $1, 8$\\
	\end{tabular}
\end{table}

For the reliability evaluation, there are different parameters to consider (Table~\ref{tab:eval_params}). For one, there are some aspects of our algorithms, that we determine just by logical reasoning and deduction. We compare them to the alternatives to verify the validity of our choice. Firstly, we use flow-based entropy measurements which need to be compared to packet-based calculations.
The mean accuracy when using packets to calculate the source port entropy reached 0.78 while the mean accuracy when calculating the entropy based on flows reaches 0.96 for all parameters. Therefore, we can conclude, that flow-based entropy measurements should be used.
Additionally, we choose the mean for combining several entropy measurements over median. Out of all test runs, in 26\% of tests, using mean to calculate the average entropy values lead to better results while in 18\% of tests, median was better. In 56\% of all cases, the results were identical. Median leads to a higher mean accuracy by 0.0005. The difference in accuracy is marginal, this confirms our choice to use mean as it takes significantly less effort to calculate.
Going forward, all reported results are using flow-based entropy, and mean for calculating the average.

The effect of the thresholds $T_h$ and $T_r$, the length of the time frames $l$ considered for the entropy evaluation and the gap length $g$ between the entropy evaluations before and during the attack are parameters dependent on requirements (\ie trade-off between precision and reaction time of the mitigation system), we analyze their respective influence on this trade-off dependent on outside influence, namely the influence of the attack strength and the start-up time of the attack. We simplify our evaluation when considering the attack start-up time in the following: For our reference value, we assume that the attack did not start yet. For the time frame where the attack is in progress, we consider different attack sizes $a$ that were reached at that specific point in time as a factor of the amount of benign UDP traffic in the network (\eg for $a = 1$, 50\% of the UDP flows in the network are attack flows). The benign traffic from and to the target has an effect on the entropy values as well (\ie entropy during an attack would be even lower when considering the benign traffic in addition to the attack traffic). For simplification, we do not consider this traffic and only consider the worst case scenario for our detection algorithm where the only traffic using the protocol used for the attack are the attackers (for the source port entropy) and the attackers are the only ones trying to access the target (for the target IP entropy). All these parameters need to be evaluated both for the UDP/TCP ratio, the destination IP entropy, and the source port entropy. DDoS attacks are aimed at a specific service hosted on one or a small amount of servers which influences the target IP entropy but does not affect the other two metrics. We analyze the target IP entropy measurements both with one server and a /29 subnet (8 servers) under attack. All in all, over 100.000 test runs were undertaken. Only a limited amount of the results can be included in this paper. In the following, we discuss the most interesting and important results of this analysis. The full analysis can be found online\footnote{https://github.com/vs-uulm/2018-DRDoS-Mitigation\_Evaluation}.

%To evaluate: destination IP entropy, source port entropy
%mixing data set with attacks of different magnitudes
%different lengths of entropy measurements
%amount of entropy measurements used
%$\Rightarrow$ classification times (table overview!)
%different $T_h$ $\Rightarrow$ $T_h$ Description needed
%attack casting times
%flow-based vs. packet-based
%mean vs. median

\begin{figure}
    \small
	\centering
	\includegraphics[width=0.92\columnwidth]{fig/udptcp.pdf}
	\caption{Precision / recall results of the UDP/TCP traffic ratio classifier with $T_r$ = [0.05, 0.1, 0.2, 0.25, 0.3, 0.35], arrow marks $T_r = 0.05$, $l=10s$, $g=60~(600s)$ (Note: Precision/Recall begins at 0.8 for better visibility; $a=0.5$ off the scale).}
	\label{fig:udp-tcp}
\end{figure}

Figure~\ref{fig:udp-tcp} shows very representative results for the UDP/TCP ratio classifier. For an attack strength $a=0.5$, precision is 90\% and recall is 78.6\% for the best $T_r$ which is too low to be within the margins of the figure.

\begin{figure}
    \small
	\centering
	\includegraphics[width=0.92\columnwidth]{fig/dip-entropy32.pdf}
	\caption{Precision / recall results of the destination IP entropy classifier for one destination IP under attack with $T_h$ = [-0.5 -1 -1.5 -2 -2.5 -3 -3.5], arrow marks $T_h = -0.5$, $l=10s$, $g=60~(600s)$ (Note: Precision/Recall begins at 0.8 for better visibility).}
	\label{fig:tip-entropy1}
\end{figure}

\begin{figure}
    \small
	\centering
	\includegraphics[width=0.92\columnwidth]{fig/dip-entropy29.pdf}
	\caption{Precision / recall results of the destination IP entropy classifier for eight destination IPs under attack with $T_h$ = [-0.5 -1 -1.5 -2 -2.5 -3 -3.5], arrow marks $T_h = -0.5$, $l=10s$, $g=60~(600s)$ (Note: Precision/Recall begins at 0.8 for better visibility; $a=0.5$ off the scale).}
	\label{fig:tip-entropy2}
\end{figure}

Figure~\ref{fig:tip-entropy1} and Figure~\ref{fig:tip-entropy2} show results for the destination IP classifier with the same parameters as for the UDP/TCP classifier. With only one server under attack (Figure~\ref{fig:tip-entropy1}), the classifier can reach usable results given a minimal attack strength of $a=1$. However, nowadays, services often are distributed over several IP addresses (Figure~\ref{fig:tip-entropy2}) which impairs the results of the IP entropy measurements. As a rule of thumb, the attack has to be twice as strong to lead to similar results for this detection scheme for a eight servers compared to one (equal distribution of attack traffic assumed).

%True positive rates not high enough to for sure say this is an attack or even a flash crowd

These result confirm, that with the right threshold (optimized for highest true positive rate) these metrics can be used as a first \emph{indicator} of an attack but not as a detection mechanism as the false positive rates are too high for a production system.

\begin{figure}
    \small
	\centering
	\includegraphics[width=0.92\columnwidth]{fig/sp-entropy1.pdf}
	\caption{Precision / recall results of the source port entropy classifier with $T_h$ = [-0.5 -1 -1.5 -2 -2.5 -3 -3.5], arrow marks $T_h = -0.5$, $l=1s$, $g=300~(300s)$ (Note: Precision/Recall begins at 0.8 for better visibility).}
	\label{fig:sp-entropy1}
\end{figure}

\begin{figure}
    \small
	\centering
	\includegraphics[width=0.92\columnwidth]{fig/sp-entropy2.pdf}
	\caption{Precision / recall results of the source port entropy classifier with $T_h$ = [-0.5 -1 -1.5 -2 -2.5 -3 -3.5], arrow marks $T_h = -0.5$, $l=90s$, $g=10~(900s)$ (Note: Precision/Recall begins at 0.8 for better visibility).}
	\label{fig:sp-entropy2}
\end{figure}

For the source port entropy, there is a clear trade-off between fast results versus correct results. For measurements with $l=600s$ and $T_h = -3.5$, an accuracy of 1 could be achieved ($g=1,~a=1$). This could not be achieved with the other metrics with any parameters at any attack strength. However, this would lead to a classification time of $900s$ which could be considered too long. With $l=10s$, accuracy can get up to $0.9996$ with a much lower classification time of $60s$ ($T=-3,~g=5,~a=4$). These results were achieved with very strong attacks. However, weaker attacks are still detectable. With $a=0.5,~l=1s,~g=3,~e=3$ and $T_h=-1$, the source port entropy can accurately decide, whether an attack is ongoing in 99.3\% of all measurements with a classification time of $4.5s$.
%TODO: results for same parameters as dest IP entropy and ratio (l,g and best T_h) l=10s g=60

A small subset of our results for the source port entropy evaluation can be seen in Figure~\ref{fig:sp-entropy1} and Figure~\ref{fig:sp-entropy2}. We chose these results as they clearly showcase the influence of the different parameters. As can be seen in both figures, the influence of $e$ is small. Taking the mean of several measurements instead of using one measurement does increase the accuracy, however, the difference is too small to justify the increase in classification time. The same can be said about the length $l$ of the entropy frames. A $1s$ frame size does suffice to reach good results. The largest influence on the results can be seen for the attack strength $a$ and the network dependent threshold $T_h$.

%Noch ein paar Worte zur Evaluation des Prototypen: Meine Testläufe liefen mit bis zu 6.5Gbps und lieferten eine sensitivity>0.99 bei der Detection (DST IP Entropie) und eine sensitivity etwas über 0,8 bei der Source Port Entropie. Durch das Queuing von Bro kam es vor, dass Angriffe erst 2g oder sogar 3g Zeitfenster nach Angriffsbeginn erkannt wurden. Zusätzlich kann ich nicht ausschließen, dass Bro bereits Pakete verworfen hat, die erst gar nicht in die Queue kamen. Meine Ergebnisse zeigen also lediglich, dass man auch bei 6.5Gbps und einem einzigen Bro-Server noch akzeptable Ergebnisse bekommt (beachte: Belwue Datensatz, Mawi Datensatz würde denke ich bessere Ergebnisse liefern). Die Evaluation ist aber absolut nicht ausgereift, d.h. man könnte meiner Einschätzung nach noch deutlich bessere Ergebnisse mit einer deutlich höheren Sicherheit bekommen. Es hat sich aber auch gezeigt, dass die Ergebnisse (sensitivity) bei allen getesteten Bandbreite sehr stabil sind und nicht abfällt. Folgendes steht zur Hardware inn der Arbeit: "The SDN controller (Ryu) and Bro are implemented by a single PC with commodity hardware: 4x3.10Ghz CPU3, 16GiB of DDR3 memory." (CPU: Intel Xeon Processor E3-1220 v3)

\subsection{Discussion}

The results show, that for one, the destination IP entropy and the UDP/TCP ratio can be good indicators for UDP-based DDoS attacks. Furthermore, the source port entropy can be used to ensure that the detected anomaly is a DRDoS attack and the mitigation mechanism can be deployed. This allows for a successful mitigation of DRDoS attacks within seconds.

Although attacks with a magnitude of $a=0.5$ can be detected most of the time, the detection system works very reliably at a magnitude $a \ge 1$. Therefore, for placement of the detection system in a network, it should be considered which attack size would be manageable by the potential target without a defense mechanism. The detector should then be placed in such a way that the usual UDP traffic going through the network node under surveillance roughly equals this maximum attack size. That way, an attack of size $a=1$ can be detected and mitigated reliably while a smaller attack might not be detected but would also not be successful.

